Hallucination In Object Detection -- A Study In Visual Part Verification

We show that object detectors can hallucinate and detect missing objects; potentially even accurately localized at their expected, but non-existing, position. This is particularly problematic for applications that rely on visual part verification: detecting if an object part is present or absent. We show how popular object detectors hallucinate objects in a visual part verification task and introduce the first visual part verification dataset: DelftBikes, which has 10,000 bike photographs, with 22 densely annotated parts per image, where some parts may be missing. We explicitly annotated an extra object state label for each part to reflect if a part is missing or intact. We propose to evaluate visual part verification by relying on recall and compare popular object detectors on DelftBikes.

==> related.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Two-stage detectors.}
Two-stage detectors consist of class-agnostic region proposals and detection parts. Early two-stage detectors \cite{girshick2015region, he2015spatial, girshick2015fast} use Selective Search algorithm \cite{uijlings2013selective} to obtain region proposals. Fast RCNN \cite{girshick2015fast} inputs the image into CNN layers and projects the ROIs onto feature map. Afterwards, it pools the region by ROI Pooling layer. Faster RCNN \cite{ren2015faster} introduces the trainable Region Proposal Network (RPN) and improves the detection accuracy and speed. Faster RCNN is a great inspiration to other detectors~\cite{dai2016r, zhu2017couplenet, lin2017feature, dai2017deformable, fan2018object, Cai_2018_CVPR, cheng2018revisiting, pang2019libra} , hence we evaluate Faster-RCNN as the prototypical two-stage detector. %the weakly-supervised object detectors \cite{kantorov2016contextlocnet}, segmentation networks \cite{shrivastava2016contextual, he2017maskRCNN}, action recognition networks \textcolor{red}{(add some references)}. 

\begin{comment}
%used ones
-RCNN\cite{girshick2015region}\\
-Spatial Pyramid Pooling (SPP-NET)\cite{he2015spatial}\\
-Fast RCNN\cite{girshick2015fast}\\
-Faster RCNN\cite{ren2015faster}\\
-Mask RCNN\cite{he2017maskRCNN}\\
-Cascade RCNN\cite{Cai_2018_CVPR}\\
-Revisiting RCNN\cite{cheng2018revisiting} and DCRv2 \cite{cheng2018decoupled}\\
-RFCN \cite{dai2016r}\\
-FPN \cite{lin2017feature}\\
-Deformable Convnet \cite{dai2017deformable}\\

-ContextLocNET\cite{kantorov2016contextlocnet}\\
-CoupleNet\cite{zhu2017couplenet}\\
-Mask Weight Network (MWN)\cite{fan2018object}\\
\end{comment}

\textbf{Single-stage detectors.}
Single-stage detectors do not use any proposal method and obtain the detection in a single run. OverFeat \cite{sermanet2013overfeat} integrates classification and localization with a single CNN.
YOLO \cite{redmon2016you} treats detection as a regression problem and predicts bounding boxes and class probabilities from a full image. In YOLOv2 \cite{Redmon_2017_CVPR} and YOLOv3 \cite{redmon2018yolov3}, the method is improved by using a deeper backbone model, multi-scale training, high resolution input and anchor boxes. 
SSD \cite{liu2016ssd} predicts category scores and box offsets for a fixed set of anchors from different scales.
RetinaNet \cite{lin2017focal} proposes focal loss which focuses on the hard training samples and provides fast convergences.
RetinaMask \cite{fu2019retinamask} extends RetinaNet with a mask prediction module and improves the performance of object detection.
EfficientDet \cite{tan2019efficientdet} scales the model and proposes fast multi-scale feature fusion to obtain better results with less parameters. For our experiments, we chose YOLOv3 and RetinaNet since they have multi-scale training and are thus comparable with Faster RCNN.


\begin{comment}
-Overfeat \cite{sermanet2013overfeat}\\
-YOLO-1\cite{redmon2016you},2\cite{Redmon_2017_CVPR},3\cite{redmon2018yolov3}\\
-SSD\cite{liu2016ssd}\\
-RetinaNET \cite{lin2017focal}\\
-EfficientDet \cite{tan2019efficientdet}\\
\end{comment}

\textbf{Context in object detection.} Before CNN-based object detectors, the role of context has been investigated by many researchers \cite{strat1993employing, oliva2001modeling, bar2004visual, luo2006pictures, hoiem2007recovering, hays2008im2gps}. Incorporating the context is studied in the aspect of co-occurrence of the context \cite{torralba2003context, rabinovich2007objects, heitz2008learning} object-to-object interactions ~\cite{wolf2006critical, murphy2004using,singhal2003probabilistic, kumar2005hierarchical}, combining different context clues \cite{divvala2009empirical} and re-scoring the detection \cite{felzenszwalb2009object}.
%Before the usage of CNNs in object detection, the role of context has been investigated by many researchers \cite{strat1993employing, oliva2001modeling, bar2004visual, luo2006pictures, hoiem2007recovering, hays2008im2gps}. Some methods \cite{torralba2003context, rabinovich2007objects} incorporate the co-occurrence of the context for detection of the objects. Some researches also consider spatial relationships between objects by using descriptors~\cite{wolf2006critical, murphy2004using}, Markov Random Fields (MRFs)~\cite{singhal2003probabilistic} and Conditional Random Fields (CRFs)~\cite{kumar2005hierarchical}. Heitz~\etal~\cite{heitz2008learning} propose a probabilistic model which links the detection of objects to unsupervised classification of relevant regions for the object. 
%Divvala~\etal~ \cite{divvala2009empirical} leverage the performance by combining different context clues.  Felzenszwalb et al. \cite{felzenszwalb2009object} use the contextual information to re-score the detection of object.
%After DL:\\
With the rise of CNNs, many approaches exploit context into a deep network. The context is exploited around the object~\cite{ gidaris2015object}, 
%RCNN  \cite{girshick2015region} crops the each object proposal from the input image with including 16 pixels context and trains each patch with AlexNet \cite{krizhevsky2012imagenet} architecture (\textcolor{red}{I am not sure if we mention this here, it can make confusion}).
as scene context~\cite{gupta2015exploring, Sun_2017_CVPR, Liu_2018, zhang2019cad}, as combinations of local parts and the global image structure~\cite{zhu2017couplenet, fan2018object} and by using multi-scale fusion and attention \cite{lim2019small}. 
Inside-Outside Net~\cite{bell2016inside} utilizes context by a recurrent neural networks. Some approaches \cite{doersch2014context, kantorov2016contextlocnet, zhang2019leveraging, xu2019hide} use the context in weakly-supervised and unsupervised \cite{doersch2015unsupervised}  object detection tasks.
%\jvg{Please group work together. I did it a bit already, but now its just an enumeration of unrelated papers, the goal is to present structure to related papers.} %\jvg{Do not write: The important work of [a] does X which is followed by the work of [b] that does Y. It has papers as the subject. Instead, make the method the subject and add citations to the method: X [a] is important, and extended by Y [b], See my writing guidelines "R1" }
%\cite{fan2018object} applies channel-wise masking on each ROI and the full feature map and combines them.
%\cite{lim2019small} proposes a SSD-based method which can detect small objects by using the context from multi-scale features.
%\cite{doersch2015unsupervised} proposes unsupervised context prediction by learning the relative location of two patches from same image.
%\textcolor{red}{(not sure if it is needed)}context in semantic segmentation \cite{yu2015multi, ghafoorian2017location}
%\cite{Sun_2017_CVPR} finds the missing curb ramps by using the context.
%? F. Yu and V. Koltun. Multi-scale context aggregation by dilated convolutions. ICLR, 2016
%-ContextLocNET\cite{kantorov2016contextlocnet}\\
%-Inside-outside net\cite{bell2016inside} **\\
%-CoupleNet\cite{zhu2017couplenet} **\\
%-Mask Weight Network (MWN)\cite{fan2018object}\\
%-Modeling visual context is key to augmenting object detection datasets (\cite{dvornik2018modeling})\\
%-Contextual Action Recognition with R*CNN \cite{Gkioxari_2015_ICCV}\\
%\textbf{Detectors discarding context:} If needed?
In addition, discarding context is studied by using a background descriptor \cite{russakovsky2012object, Cinbis_2017} and contrast-based scoring \cite{Cho_2015_CVPR}. To have a robust decision, \cite{zhang2019bag} uses mixup augmentation and \cite{singh2020don} investigates how to disentangle object from its co-occurring context.
% \jvg{ no new paragraph unless a new topic is mentioned. Group papers by similar approach/topic, where 'similar' is defined by how you think they should be grouped(\textcolor{red}{they try to discard the context})}, %\cite{russakovsky2012object, Cinbis_2017} use a background descriptor to model background and help the detection model to be aware of objects and their context. Cho et al. \cite{Cho_2015_CVPR} present a contrast-based contextual score between a ROI and its surrounding area for unsupervised localization.
 %\cite{zhang2019bag} uses mixup augmentation for object detection and results in more robust detection in incoherent context, like elephant in the room \cite{Rosenfeld2018TheEI}.  
%\cite{singh2020don} investigates how to disentangle object from its co-occurring context for classification task and to be more robust against contextual biases.
%- Weakly Supervised Object Localization with Multi-fold Multiple Instance Learning :we have presented a contrastive background descriptor, which encourages the detection model to learn the differences between the objects and their context \cite{Cinbis_2017}\\
% O. Russakovsky, Y. Lin, K. Yu, and L. Fei-Fei. Object-centric spatial pooling for image classification. In European Conference on Computer Vision, 2012 : Foreground-Background Feature Representation (i am not sure) \cite{russakovsky2012object} \\
%From contextloc : Russakovsky et al. [29] and Cinbis et al. [2] use a background descriptor computed over features outside a candidate box, and demonstrate that background modelling can improve WSL as compared to foreground modelling only. \\
%\cite{Cho_2015_CVPR}propose a contrast-based contextual score for unsupervised object localization, which measures the contrast of matching scores between a candidate region and its surrounding candidate regions.\\
%\textbf{Similar to ours:}
%\textcolor{red}{(improve this part)} \jvg{include in the grouping}
%-Putting visual object recognition in context\cite{zhang2019putting}\\
\cite{zhang2019putting} investigates the contextual effect on visual recognition with different ways and compare with human performance.
%-Exploring the Bounds of the Utility of Context for Object Detection \cite{Barnea_2019_CVPR}
%\textcolor{red}{(Is the context general or only ob-to-obj?)}
\cite{Barnea_2019_CVPR} explores the bounds of object classes by using contextual information and show the cases when is beneficial to use or discard. 
%\textcolor{red}{(show here our differences from them)}
In this paper, we explain why object detectors hallucinate by an aspect of context. The effect of context is shown extensively
%as class-specific results and
on overall performances on different types of deep object detectors and the detector performances and their failure cases are compared on COCO and BikeParts dataset.
%MICS
\begin{comment}



**3. [Exploring the Bounds of the Utility of Context for Object Detection](https://arxiv.org/pdf/1711.05471.pdf)





-12. [Bottom-up Object Detection by Grouping Extreme and Center Points](https://arxiv.org/pdf/1901.08043.pdf)


14. [A Survey of Deep Learning-based Object Detection](https://arxiv.org/pdf/1907.09408.pdf)

20.[ Speed/accuracy trade-offs for modern convolutional object detectors](https://arxiv.org/pdf/1611.10012.pdf) (especially citations about Faster rcnn type detectors)


\end{comment}

\begin{figure}
	\centering
	%\begin{tabular}{c@{}c}
	\includegraphics[width=0.99\linewidth]{images/object_states_dist.pdf}
	%images/white_bg_complete_intact.png}
	%\end{tabular}
	\caption{The distribution of part states for train and test sets. For both train and test sets, intact parts has the highest ratio by 60\%. Approximately 20\% of parts in the dataset are absent.}
	%{The distribution of part states for entire dataset. For essential parts like front wheel, back wheel and steer, the dataset has high intact rate and lower absent or occluded states. For optional parts such as bell, dynamo and dressing guard, the number of absent state is higher than intact states.}
	\label{fig:states}
\end{figure}
